UI-Vision: A Desktop-centric GUI Benchmark for Visual Perception and Interaction

Autonomous agents that navigate Graphical User Interfaces (GUIs) to automate tasks like document editing and file management can greatly enhance computer workflows. While existing research focuses on online settings, desktop environments, critical for many professional and everyday tasks, remain underexplored due to data collection challenges and licensing issues. We introduce UI-Vision, the first comprehensive, license-permissive benchmark for offline, fine-grained evaluation of computer use agents in real-world desktop environments. Unlike online benchmarks, UI-Vision provides: (i) dense, high-quality annotations of human demonstrations, including bounding boxes, UI labels, and action trajectories (clicks, drags, and keyboard inputs) across 83 software applications, and (ii) three fine-to-coarse grained tasks-Element Grounding, Layout Grounding, and Action Prediction-with well-defined metrics to rigorously evaluate agents' performance in desktop environments. Our evaluation reveals critical limitations in state-of-the-art models like UI-TARS-72B, including issues with understanding professional software, spatial reasoning, and complex actions like drag-and-drop. These findings highlight the challenges in developing fully autonomous computer use agents. By releasing UI-Vision as open-source, we aim to advance the development of more capable agents for real-world desktop tasks.

==> sections/rebuttal_titling.tex <==
\twocolumn[
\icmltitle{\texorpdfstring{
\raisebox{-.6ex}{\includegraphics[width=0.6cm]{figures/icons/square.png}}\,
Rebuttal Material for \dataset}{UI-Vision: A Desktop-centric GUI Benchmark for Visual Perception and Interaction}}
% It is OKAY to include author information, even for blind
% submissions: the style file will automatically remove it for you
% unless you've provided the [accepted] option to the icml2025
% package.
% List of affiliations: The first argument should be a (short)
% identifier you will use later to specify author affiliations
% Academic affiliations should list Department, University, City, Region, Countrygg
% Industry affiliations should list Company, City, Region, Country
% You can specify symbols, otherwise they are numbered in order.
% Ideally, you should not use this facility. Affiliations will be numbered
% in order of appearance and this is the preferred way.
\icmlsetsymbol{equal}{*}
\begin{icmlauthorlist}
\icmlauthor{Shravan Nayak}{equal,mila,udem,snow}
\icmlauthor{Xiangru Jian}{equal,uw,snow}
\icmlauthor{Kevin Qinghong Lin}{nus}
\icmlauthor{Juan A. Rodriguez}{mila,snow,ets}
\icmlauthor{Montek Kalsi}{snow}
\icmlauthor{Rabiul Awal}{mila,udem,snow}
\icmlauthor{Nicolas Chapados}{snow}
\icmlauthor{M. Tamer Özsu}{uw}
\icmlauthor{Aishwarya Agrawal}{mila,udem,cifar}
\icmlauthor{David Vazquez}{snow}
\icmlauthor{Christopher Pal}{mila,poly,snow,cifar}
\icmlauthor{Perouz Taslakian}{snow}
\icmlauthor{Spandana Gella}{snow}
\icmlauthor{Sai Rajeswar}{snow,mila,udem}
\end{icmlauthorlist}

\icmlaffiliation{mila}{Mila - Quebec AI Institute}
\icmlaffiliation{udem}{Université de Montréal}
\icmlaffiliation{uw}{University of Waterloo}
\icmlaffiliation{snow}{ServiceNow}
\icmlaffiliation{nus}{National University of Singapore}
\icmlaffiliation{poly}{Polytechnique Montréal}
\icmlaffiliation{cifar}{CIFAR AI Chair}
\icmlaffiliation{ets}{École de Technologie Supérieure}
\icmlcorrespondingauthor{Shravan Nayak}{shravan.nayak@mila.quebec}
\icmlcorrespondingauthor{Xiangru Jian}{x2jian@uwaterloo.ca}
% You may provide any keywords that you
% find helpful for describing your paper; these are used to populate
% the "keywords" metadata in the PDF but will not be shown in the document
\icmlkeywords{Agents, GUI, Large Language Models, Vision Language Models, Multimodality}
\vskip 0.3in
]

% this must go after the closing bracket ] following \twocolumn[ ...

% This command actually creates the footnote in the first column
% listing the affiliations and the copyright notice.
% The command takes one argument, which is text to display at the start of the footnote.
% The \icmlEqualContribution command is standard text for equal contribution.
% Remove it (just {}) if you do not need this facility.

%\printAffiliationsAndNotice{}  % leave blank if no need to mention equal contribution
\printAffiliationsAndNotice{\icmlEqualContribution} % otherwise use the standard text.
